Message Passing and Combinatorial Optimization

Graphical models use the intuitive and well-studied methods of graph theory to implicitly represent dependencies between variables in large systems. They can model the global behaviour of a complex system by specifying only local factors. This thesis studies inference in discrete graphical models from an algebraic perspective and the ways inference can be used to express and approximate NP-hard combinatorial problems. We investigate the complexity and reducibility of various inference problems, in part by organizing them in an inference hierarchy. We then investigate tractable approximations for a subset of these problems using distributive law in the form of message passing. The quality of the resulting message passing procedure, called Belief Propagation (BP), depends on the influence of loops in the graphical model. We contribute to three classes of approximations that improve BP for loopy graphs A) loop correction techniques; B) survey propagation, another message passing technique that surpasses BP in some settings; and C) hybrid methods that interpolate between deterministic message passing and Markov Chain Monte Carlo inference. We then review the existing message passing solutions and provide novel graphical models and inference techniques for combinatorial problems under three broad classes: A) constraint satisfaction problems such as satisfiability, coloring, packing, set / clique-cover and dominating / independent set and their optimization counterparts; B) clustering problems such as hierarchical clustering, K-median, K-clustering, K-center and modularity optimization; C) problems over permutations including assignment, graph morphisms and alignment, finding symmetries and traveling salesman problem. In many cases we show that message passing is able to find solutions that are either near optimal or favourably compare with today's state-of-the-art approaches.

==> appa.tex <==
\begin{comment}
\chapter{Appendix A}
\section{Expectation Propagation}\label{sec:ep}

\refCite{Minka2001,Minka2005} introduced Expectation Propagation
 as an extension of Assumed Density Filtering: a generalization of Kalman Filter to deal
with  messages that are arbitrary functions, by projecting them to tractable
class of distributions (\refCite{Opper1998}). This projection is performed by
maximum likelihood estimation (or matching of sufficient statistics, \aka moment
matching) or in general minimization of an $\alpha$-divergence
measure (see \refEq{eq:alphadivergence}).

EP generalized many known algorithms, in ways that
provided complementary perspective to that of variational free-energy
minimization. To appreciate the connection we first overview the basic form of
EP.

EP is an iterative refinement procedure in which a particular distribution of
interest
\begin{align}
\p(\x) \quad = \quad \q(\x) \prod_{\I{I}} \f_{\I{I}}(\x_{\I{I}})   
\end{align} 
depends on some intractable ($\f_{\I{I}}$) functions-- that is we can not
exactly incorporate these factors into $\p$'s parametric representation.
$\q(\x)$ is the tractable part.

To represent this product form, EP iteratively updates a parametric form
$\ph(\x, \params)$ so as to best incorporate $\f_{\I{I}}$ within its parametric
family:
\begin{enumerate}\label{env:ep}
  \item Start with $\ph(\x, \params) \; = \; \q(\x)$ and
  $\fh_{\I{I}}(\x_{\I{I}}; \param_{\I{I}}) \;=\; \set{U}(\x)$ (or some other
  initialization).
  $\fh_{\I{I}}(\x_{\I{I}}; \param_{\I{I}})$'s are going to be refined and in the
   end represent $\f_{\I{I}}$ within the tractable family of our interest. 
   Note that here $\param_{\I{I}}$ is not a sub-vector of
  $\params$; Here it instead defines $\fh_{\I{I}}$.
  \item Until convergence (successive $\params$ are approximately equal):
  \begin{enumerate}
    \item Choose a function index $\I{I}$.
    \item Remove previously incorporated factor ${\fh_{\I{I}}(\x_{\I{I}};
    \param_{\I{I}})}$:
   		\begin{align}
   			\ph_{\back \I{I}} \quad \propto \quad \frac{\ph}{\fh_{\I{I}}}  
   		\end{align}
    \item  Solve the maximum likelihood problem: 
    \begin{align}\label{eq:eplikelihood}
    \params^* \quad = \quad \arg_{\params^*}\min \quad \set{D}_{KL} \left (
    \ph_{\back \I{I}}(\x, \params)
    \f_{\I{I}}(\x_{\I{I}}) \;,\;
    \ph(\x, \params^*)
    \right )
    \end{align}
    
    \item Update $\param_{\I{I}}$ such that:
    	\begin{align}
    	\fh_{\I{I}}(\x_{\I{I}}; \param_{\I{I}}) \quad \propto \quad 
    	\frac{\ph(\x,\params^*)}{\ph_{\back \I{I}}(\x, \params)} 
    	\end{align}
    \item Set $\params = \params^*$
   \end{enumerate}
\end{enumerate}

This update procedure reduces to BP when $\ph(\x, \params)$ has a completely
decomposable form-- \ie $\params = [\param_i]_i$ and $\f_{\I{I}}$ are PGM's
factors, which can not be directly included in the product form representation
of $\ph(\x, \params)$.

\subsubsection{ Local versus Global Divergence Minimization}
From variational perspective of previous section, all well-known inference
algorithms are minimizing an approximate form of exclusive KL-divergence
$\set{D}(\ph, \p)$ to find $\ph$. \emph{However the only optimization that
produces marginals and correct integrals (\eg partition function) is the inclusive
minimization of KL-divergence $\set{D}(\p, \ph)$ wrt $\ph$.} This role reversal
is because of computational convenience: as we do not have access to $\p$, it
is difficult to calculate expectations based on it. 

However EP gives us a different perspective. \emph{The local divergence
minimization of \refEq{eq:eplikelihood} can be replaced with any other $\alpha$-divergence,
and the EP algorithm above is an attempt to optimize the corresponding global
divergence measure.} 

$\alpha$-divergence for unnormalized distributions $\p$ and
$\ph$ has the following form (\refCite{Amari1985}):
\begin{align}\label{eq:alphadivergence}
\set{D}_{\alpha}(\p | \ph) \quad = \quad \frac
{\int_{\x} \alpha \p(\x)\; + \; (1-\alpha) \ph(\x) \; -\;
\p(\x)^{\alpha}\ph(\x)^{1-\alpha} \; d\x} {\alpha (1 - \alpha )} \quad ,\quad
\alpha \in (-\infty, \infty)
\end{align}
which reduces to $\set{D}(\p, \ph)$ and $\set{D}(\ph, \p)$ at the limit of
$\alpha = 1$ and $\alpha = 0$ respectively. 

Based on this view, BP is
attempting to minimize the inclusive KL-divergence (see \refEq{eq:eplikelihood}). 
At first this may seem contradictory as we have derived BP
equations as minimizers of exclusive KL-divergence in \refSection{sec:bpagain}.
However, we can resolve the contradiction by simply realizing that the two
models that are being used are different. 
In variational derivation we used a parametric form
similar to \refEq{eq:treereparam} for $\ph$ while using EP, $\ph$ is assumed to
have a completely decomposable form $\ph(\x; \params) \propto \prod_{i} \ph(\x_i, \param_i)$. 

Another consequence of this perspective is that the naive mean field is
minimizing exclusive divergence. We can derive mean field by replacing the error
measure of \refEq{eq:eplikelihood} with exclusive KL-divergence. In fact Minka
shows that among all the $\alpha$-divergences, only for exclusive KL-divergence,
local minimization is exactly the same as global minimization of
divergence\footnote{This is not to be confused with having local and global
optima. In both cases a coordinate ascend method such as MF gets trapped in
local optima.}.

The general form of EP for arbitrary $\alpha$ is called ``power EP''
(\refCite{Minka2004}), which reduce to Fractional
BP (\refCite{Wiegerinck2003}), variational message passing-- a message passing
form of naive MF (\refCite{Winn2005}) and Tree-Reweighted BP
(\refCite{Wainwright2005a}) for different choices of $\alpha$.

EP also has been applied to more expressive distributions than the ones with
product form. By considering $\ph(\x, \params)$ to be a distribution over an
spanning tree --that includes a subset of factors of our PGM-- we get the better
approximation of Tree EP method (\refCite{Minka2002}).

EP too can be expressed in variational perspective. The energy minimized by EP
and its constraint optimization is discussed in several sources
(\refCite{Minka2005,Koller2009}). In particular
\refCite{Wainwright2007} gives an interesting and comprehensive account. 
The connection between EP and region-based methods is established in
\refCite{Welling2005}. Finally \refCite{MinkaWeb} provides references to
various applications of EP in different domains.
\end{comment}
\section{Replica trick}
\begin{comment}
The replica trick is a mathematical trick that is used to estimate the
self-averaging quantities in spin-glass theory and combinatorial optimization.
In particular it is used to estimate the average free energy and overlap
distribution. Here we show in a nutshell how it is used to calculate
average free energy. Then we consider using this trick in practice.

Free
energy can give us valuable information about the system of interest. 
For example its local optima gives us meta-stable states 
(\ie the sub-measures of Gibbs measure over the system) 
and its global optima at zero temperature produces the
ground states of the system.

However, calculating the average of \refEq{eq:freeenergy2}:
\begin{align}
\overline{\F_{\ns}(\f)} \quad = \quad \int_{\f}  \frac{1}{\ns \beta}\log \left ( \int_{\x \in \set{X}}
\expp{-\beta \sum_{\I{I}}\f_{\I{I}}(\x)} \right ) d\x 
\end{align}
is a difficult task. If the logarithm was outside the outer integral this
calculation would have been easier, as we were averaging over all possible
states and realizations of PGM at the same time. This is known as the annealed
average and is not what we really want! 

In many attempts to solve the SK model -- \ie to analyze its behaviour--
 a trick was employed to calculate average free energy.
The idea is to use the following expansion:
\begin{align}
\Z_{\ns}^{d}(\f) \quad = \quad 1 + d \log(\Z_{\ns}(\f)) + \set{O}(d^2)
\end{align}
which after some calculation gives:
\begin{align}
\overline{\F_{\ns}(\f)} \quad = \frac{1}{\ns
\beta} \quad \overline{\log(\Z)} \quad = \quad \lim_{d
\to 0} \frac{1}{\ns
\beta} \frac{1}{d}\log(\overline{\Z^d} )
\end{align}
Here $\Z^d$ is equal to the partition function of $d$ replicates of the original
system, hence the name ``replica trick''. Here we are calculating the average of
free energy by calculating the average of the partition function of  $d$
replicates of the system, and then (unexpectedly) taking the limit of $d$ to
zero. Although important results have been obtained using this trick,
mathematically it is not well-founded at the thermodynamic limit
(\refCite{Mezard1987}).
An alternative approach to calculate self-averaging properties is so
called ``cavity method'', which is more involved and mathematically more
rigorous but it is found to give identical results (\eg \refCite{Mezard2009}).
\end{comment}


==> appc.tex <==
\chapter{Bioinformatics and handwriting/speech recognition: unconventional applications of similarity search tools}
\section{Introduction}
	Bioinformatics has benefited immensely from tools and techniques imported
	from other disciplines.  Markov models used for gene--finding have
	their origin in information science, neural networks are imported
	from machine learning, and the countless clustering methods used
	for analyzing microarray data are from a wide variety of fields.

	Sequence alignment tools are no exception to this trend;
	however, within bioinformatics, they have reached
	new levels of speed and sophistication.  Tools,
	such as Blast~\cite{altschul1990basic,altschul1997gapped}
	and FastA~\cite{pearson1998improved}, are used routinely to search
	through a database for sequences (DNA or protein) that are
	similar to a query sequence.  Over the years, these tools have
	been optimized for speed by employing a number of heuristic
	shortcuts to the dynamic programming algorithms on which
	they are based.  Even searches in very large databases,
	such as Swiss--Prot/TrEMBL~\cite{bairoch2000swiss-prot} or
	GenBank~\cite{benson2000genbank}, take only a few seconds
	for queries of small to moderate size.	This is substantially
	faster than the time required for a rigorous Smith--Waterman
	search~\cite{waterman1984efficient}.  In light of the remarkably
	speed and accuracy that characterize these algorithms, it is 
	intriguing to investigate other applications where similarity
	search tools might be of material importance.  In this work, we present two
	alternative applications of these fast sequence alignment tools
	outside the domain of bioinformatics: handwriting recognition and
	speech recognition.

	The dynamic handwriting recognition problem is to recognize
	handwriting from a touch tablet as found on personal
	digital assistants (PDAs), for example Palm Pilots, or tablet
	PCs~\cite{tappert1990thestate}.  These writing tablets sample
	the position of a pen as a function of time to produce a series of
	($x,y$) points that are used by handwriting recognition algorithms to
	determine which character was written.	An excellent review of the
	most common algorithms is available from Plamodon and Srihari, 2000.
	These include feature analysis, curve matching, Markov models, and
	elastic matching, the last of which is based on dynamic programming
	and is related to both Blast and FastA.

	To apply similarity search concepts to the handwriting recognition
	problem, we represented the path of a PDA pen as a protein
	sequence by translating the ($x,y$) points into a string of
	amino acids.  Using the protein representation of handwriting
	samples, we were able to classify unknown samples with FastA. 
	This is analogous to the problem of protein annotation using
	similarity searching: given a protein (a written character)
	of unknown function, we annotated the protein by searching for
	similar sequences (characters with similar ($x,y$) paths).

	We applied the same sequence alignment approach to speech
	recognition.  Automated phone services, security checkpoints,
	and computer dictation software employ some form of speech
	recognition.  Common speech recognition methods include feature
	recognition, neural networks, hidden Markov models, dynamic
	programming~\cite{ney2000progress} and a variety of other statistical
	and signal processing algorithms.  A good review of these techniques
	and more is available from Juang \& Furui, 2000.  For this problem,
	we represented digital speech recordings as sequences of amino
	acids, and used a database of annotated recordings to classify
	unknown recordings.

	In the following section, we describe the data sets used for the
	handwriting recognition and speech recognition problems.  Then,
	we detail how these data were represented using strings of amino
	acids and how we used FastA to annotate unknown samples in four
	handwriting and speech recognition experiments.  We compare our
	results to more traditional methods of handwriting and speech
	recognition and, finally, we discuss ways of improving upon the
	results and extending sequence alignment to other classification
	problems.

		\begin{figure}[t!]
				\centering
				\includegraphics[width=\textwidth]{Images-appc/digits.pdf}
			\caption{Projection of a digit written with
					a PDA stylus into protein space.
					Concatenating the set of
					points gives a protein sequence
					representative of the digit.
					In this case, the sequence is
					\texttt{QYKXVVFMWGSNHANQ}.%
					An alignment of nines from two
					different writers.  The boxes at
					the top show the input from each
					writer and the large grid show the
					superposition of the two handwritten
					digits.  The FastA alignment between
					the protein representations of the
					two digits is shown in the center.
				Two visualizations of the handwriting
				recognition problem.  In both cases the
				$x$ and $y$ axes are divided into 23 parts
				corresponding to the columns and rows in
				an amino acid scoring matrix.  The eight
				sampled points from the digit are cast from
				$x,y$ space into protein space by assigning
				amino acid coordinates to each point.
			}\label{fig:pda}\label{fig:pdaAlign}
		\end{figure}

		\begin{table*}[t!] 
			\centering
			\caption[fooba]{Results for the handwriting and
				speech recognition problems described
				in the text.  For each experiment,
				the misclassification is the percent of
				sequences in the unknown set for which the
				digit or letter was not predicted correctly.}
			\subtable[
				Handwriting recognition results.
			]{\input{Images-appc/table_results1}} \subtable[Speech
				recognition results.
				The second column shows the
				misclassification using the clustering of
				all /ee/ sounding letters as described in the
				text.  ]{ \input{Images-appc/table_results2} }
			\label{table:results2}\label{table:results1}
		\end{table*}


		\begin{table*}[!b]
		\centering
		\caption[Handwriting Alignment Scoring Matrix]{The scoring matrix used for the handwriting
			and speech recognition FastA alignments.
			Each entry of the scoring matrix, $s_{ij}$, is given by $s_{ij}= 10-(|i-j|)$.
			That is, matching amino acids are given 10 ``points'', amino acids
			that are one off are given 9 points, and so on.  This matrix was used
			in place of the default scoring matrix,  Blosum50~\cite{henikoff1992aminoacid},  for FastA.
			The scoring matrix was found heuristically.  Also, a few experiments indicated that the
			alignments are relatively insensitive to permutations about the form of $s_{ij}$ given above.

		} \label{table:matrix}
		\include{Images-appc/table_matrix}
		\end{table*}

		\begin{figure}[ptbh]
		\centering
		\includegraphics[width=\textwidth]{Images-appc/voice.pdf}
		
			%\scalebox{0.80}{
			%	\footnotesize
			%	\input{Images-appc/fig_voiceAlign}
			%	\normalsize
			%}
		\caption[A Voice alignment]{
			An alignment of the spoken--letter ``X'' recorded from two different speakers.
			The plots at the top and bottom are recordings for first and second
			speakers, respectively.  The breakout in the center shows a section of the protein
			projection of each recording and the alignment generated using FastA
			as described in the text.  This example was taken from the first speech
			recognition experiment.  In this case, the bottom recording was the top
			scoring alignment against the top recording.
		}
		\label{fig:voiceAlign}
		\end{figure}

		\begin{figure}[ptbh]
		\centering
		\includegraphics[width=\textwidth]{Images-appc/tree.pdf}
		\caption[A PDA digit]{
			A phylogenetic tree of voice--proteins.
			This tree was created using the
			Phylip~\cite{felsenstein1989phylip} tree drawing
			program from a multiple sequence alignment of
			all 26 voice--proteins from a single speaker.
			The multiple sequence alignment was made using the
			ClustalW~\cite{higgins1992improved} alignment tool,
			with the scoring matrix in Table~\vref{table:matrix}.
			In the tree, similar sounding (homologous) letters
			are grouped near each other.  For example, all the
			letters containing the /ee/ sound [\emph{B, C, D,
			E, G, P, T, V, Z}] are clustered on the left side
			of the tree.
		} \label{fig:tree} \end{figure}



\section{System and Methods}
	\subsection{Handwriting Recognition}
		For our handwriting recognition experiments, we used
		data from Alimoglu and Alpaydin, 1996, available in the
		University of California Irvine repository of machine
		learning databases~\cite{uci1998ucirepository}.  These data
		comprised of 10992 handwritten digits between \emph{0}
		and \emph{9}, written by 44 writers with each writer
		submitting 250 digits (8 samples were discarded by the
		original authors).

		Each digit was written with a stylus pen on a touch tablet,
		which recorded the $x$ and $y$ coordinates of the pen as a
		function of time.  These data were re-sampled such that each
		written digit was represented by a series of eight $(x,y)$
		points, spaced out by a constant arc length over the path of
		the digit.  Then, for each digit, the set of $(x,y)$ points
		were scaled such that the largest axis, usually the $y$ axis,
		ranged from 0 to 1.  By dividing the number line $[0,1]$
		into 23 ``bins'' we translated each of these coordinates
		into a pair of amino acids as shown in Figure~\vref{fig:pda}.
		We concatenated these amino acid pairs to obtain a protein
		sequence representation of each digit: a ``digit--protein.''



		
	\subsection{Speech Recognition}
		For our speech recognition experiments, we used data from
		Deitterich and Bakiri, 1995, %~\cite{dietterich1995solving}
		available in the University of California Irvine repository
		of machine learning databases~\cite{uci1998ucirepository}.
		This data set consisted of 7797 recordings of individuals
		speaking one of the letters \emph{A--Z}.  A total of 150
		speakers each said every letter \emph{A--Z} twice (three
		recordings were discarded by the original authors).
		Then, each recording was processed into a set of 617
		real--valued attributes in the range $[-1,1]$.	A more
		detailed description of the database is available from
		Dietterich \& Bakiri, 1995.%~\cite{dietterich1995solving}.

		By dividing the number line $[-1,1]$ into 23 bins we translated these real numbers into a series
		of amino acids.  For example, the series ``-1.0,-0.55, 0.11, 0.65'' was translated
		to ``{\texttt{AQKY}}''.  We concatenated these amino acids to make a protein representation
		of each recording: a ``voice--protein''.


\section{Results}
	\subsection{Handwriting Recognition}

		We conducted two handwriting recognition experiments.
		In both experiments part of the digit--protein database was assumed to contain a
		``known'' set of digits that was subsequently used to annotate,
		or classify, the remaining ``unknown'' digits.	For our
		first experiment, we used for the known database containing the
		writing of 30 persons (7494 digits) and an unknown database
		with the writing of the remaining 14 persons (3498 digits).
		Using FastA, we searched each sequence from the unknown
		set in the known set and used the top scoring hits to
		annotate the unknown digits.  Searches were carried out
		using the scoring matrix shown in Table~\vref{table:matrix}
		with FastA version 3.4t11 using the default gap open and
		extension penalties, and the following options: \texttt{-p
		-Q -d0 -f-8 -g-1 -H -E1000 -b1}.  An example alignment of
		two handwritten nines from different writers is shown in
		Figure~\vref{fig:pdaAlign}.


		For our second experiment, we used 25\% (2748 digits) of our
		digit--protein database, selected randomly, as the unknown
		set and the remaining 75\% (8244 digits) as our known set.
		Alignments and annotations using FastA were performed as
		in the first experiment.

		The results of the two handwriting recognition
		experiments are shown in Table~\vref{table:results1}.
		In experiment 1, our results are about the same as
		the best k--means clustering results of Alimoglu and
		Alpaydin~\cite{alimoglu1996methods,alimoglu1997combining}.
		This experiment simulates the user--independent
		handwriting recognition problem: the handwriting of one
		group of writers was used to classify digits from a different group.
		In the user--dependent problem, experiment 2, the database
		of known handwritten digits contains samples from all the writers,
		on average.  Thus, for every unknown handwriting sample,
		there is often a close match in the database of known
		samples.  As such, the results of experiment 2 are
		significantly better than those of experiment 1 as shown
		in Table~\vref{table:results1}.



		%In contrast to k--means clustering and other common machine learning techniques for handwriting
		%recognition, there was no explicit training or learning phase of our experiments.  As such, 
		%we included experiment 3, which is a realistic approximation of the recognition problem 
		%on a tablet PC with multiple users.  The results for this experiment are considerably better than
		%experiment 2 because there are relatively more known sequences which can be used for annotating
		%the unknown sequence.

		In experiment 1, the average time for each alignment was
		0.117 seconds per unknown sequence on a 1 gHz Pentium III
		processor.  This is much shorter than the time required to
		write the digits.  Thus sequence alignment could be used
		as a ``real--time'' method for handwriting recognition.
		This high speed, together with the high accuracy for
		user--dependent recognition makes sequence alignment good
		candidate for use on a Tablet PCs, or even PDAs.

	\subsection{Speech Recognition}


		Using the voice--protein database, we conducted two
		experiments, analogous to the two handwriting recognition
		experiments described previously.  First, we used a known
		set consisting of 6238 recordings from 120 speakers and
		an unknown set with 1559 recordings from the remaining 30
		speakers.  Second, we used 25\% (1949 recordings) of the
		voice--protein database, selected randomly, as the unknown
		set and the remaining 75\% (5848 recordings) as the known
		set.  Each of the speech recognition alignments was performed
		using the same scoring matrix and FastA parameters as the
		handwriting recognition experiments.  An example alignment
		of two voice--proteins is shown in Figure~\vref{fig:voiceAlign}.


		The results of the two speech recognition experiments are shown in
		Table~\vref{table:results2}.
		Experiment 1 is compared
		to the best Error Correcting Output Code (ECOC) results of Deitterich
		and Bakiri,
		%~\cite{dietterich1995solving}
		but
		there was no comparison available for experiment 2.	
		The misclassification for experiment 1 was 6.16\%, 
		higher than the ECOC result of 3.27\%.  However, we observed that
		most of the errors were due to rhyming letters, and in particular
		all of the /ee/ sounding characters [\emph{B, C, D, E, G, P, T, V, Z}].
		This indicated that these characters were similar on a sequence level,
		so we constructed a phylogenetic tree of the sequences to study their
		relationship.

	

		A phylogenetic tree of 26 voice--proteins from a single
		speaker is shown in Figure~\vref{fig:tree}.  As the figure
		shows, the protein projections of phonetically similar
		letters tend to be homologous.	Furthermore, letters such
		as \emph{A} and \emph{H}, which have the /ay/ sound at the
		beginning, are more closely related to each other than
		they are to \emph{J} and \emph{K}, which have the /ay/
		sound at the end.  Because the /ee/ sounding letters all
		have /ee/ at the end, they are particularly difficult
		to distinguish from each other.  These letters account
		for a disproportionate majority of the errors in our two
		experiments.  By clustering these letters together such that
		they are considered the same for classification purposes,
		the error in experiment 1 was reduced to 1.09\%.  If the
		original error was evenly distributed between the classes,
		the error would have been reduced only to about 5.5\%.
		This suggests that, although string alignment performs
		poorly for /ee/ sounding characters, it performs well for
		all other characters.


\section{Conclusions}
		This work showed that sequence alignment can be a powerful
		classification tool for problems outside the domain
		of bioinformatics.  In both the handwriting and speech
		recognition problems, we projected real--valued data into
		strings of amino acids and used FastA as a classification
		tool, in a manner analogous to protein annotation.  In the
		case of handwriting recognition, we showed that sequence
		alignment is a viable alternative to traditional methods,
		such as k--means clustering, and is fast enough to be used
		as a real--time recognition method.


		There are many ways to improve upon the results we presented here.
		First, we did not have any explicit training phase for either set of experiments.
		However, there are at least two sequence alignment parameters which can
		be trained: the gap open and extension penalties, and the scoring matrix.
		The optimization of these parameters for protein annotation is well documented
		~\cite{henikoff1993performance,altschul1991amino,henikoff1992aminoacid,dayhoff1979amodel,vogt1995assessment,henikoff2000amino}
		and would be similar for alternative sequence alignment applications such
		as handwriting recognition.  Second, intelligent projection of data
		into strings can greatly improve results.  Here, we used bins of equal
		size to partition the real--valued data into amino acids; however, bins
		of unequal size may improve the resolution between closely related sequences
		and improve classification.  Finally, more customizable sequence alignment tools
		would be very useful.  These tools should take an arbitrary alphabet (Blast
		and FastA are restricted to 23 amino acids) and a user--defined scoring
		matrix (FastA allows user--defined matrices, but Blast does not).

		The potential applications of sequence alignment tools
		outside of bioinformatics are boundless.  Tools such as Blast
		and FastA can be used to quickly classify or search through
		any data that can be projected into a string of characters.
		Of course, these methods will work best with data that is
		of a low dimension.  Our experiments with more complex data
		data, such as color images, suggest that how the data are
		projected into a string is very important with large number
		of dimensions.	However, for simple types of data, such
		as customer purchase histories, black and white images, or
		Internet chat transcripts, we have been able to use sequence
		alignment as a quick and effective classification tool.



==> bpb.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 

\begin{comment}
\subsection{Gibbs Sampling as Message Update}\label{sec:gs}
Gibbs Sampling (GS) is a Markov Chain Monte Carlo (MCMC) inference
procedure (\refCitep{Andrieu2003}) that can produce a set of samples
$\xh[1], \ldots, \xh[L]$ from a given PGM. We can then recover the
marginal probabilities, as empirical expectations:
\begin{align}\label{eq:empavg}
  \ph^{L}(\x_i) \quad \propto \quad \frac{1}{L} \sum_{n=1}^{L}
  \delta(\xh[{n}]_i,\x_i)
\end{align}

Our algorithm only consider a single particle $\xh = \xh[1]$.  GS starts
from a random initial state $\xh\nn{t = 0}$ and at each time-step $t$,
updates each $\xh_i$ by sampling from:
\begin{align}\label{eq:gs}
  \xh\nn{t}_i \; \sim \; \p(\x_i) \quad \propto \quad \prod_{I
    \in \partial i} \f_{I}(\x_i , \xh^{(t-1)}_{\partial I \back i})
\end{align}

If the Markov chain satisfies certain basic properties
(\refCitep{casella1999monte}), $\x_i\nn{\infty}$ is guaranteed to be
an unbiased sample from $\p(\x_i)$ and therefore our marginal
estimate, $\ph^L(\x_i)$, becomes exact as $L \to \infty$.

In order to interpolate between BP and GS, we establish a
correspondence between a particle in GS and a set of variable-to-factor 
messages --\ie $\xh \Leftrightarrow \{\Ms{i}{I}(.)\}_{i, I
  \in \partial i}$.  Here all the messages leaving variable $\x_i$ are
equal to a $\delta$-function defined based on $\xh_i$:
\begin{align}
  \Ms{i}{I}(\x_i) \; = \; \delta(\x_i, \xh_i) \quad \forall I
  \in \partial i
\end{align}

We define the random GS operator $\gs = \{ \gsi{i}\}_i$
and rewrite the GS update of \refEq{eq:gs} as
\begin{align}\label{eq:gsop}
  \Ms{i}{I}(\x_i) \quad \triangleq \quad  \gsi{i}(\{\Ms{j}{J}(\x_j) \}_{j \in
    \mb i, J \in \partial i})(\x_i) \quad = \quad \delta(\xh_i, x_i)
\end{align}
where $\xh_i$ is sampled from
\begin{align}
  \xh_i \; \sim \; \ph(\x_i)  \quad &\propto \quad \prod_{J \in \partial i}
  \f_{I}(\x_i , \xh_{\partial I \back i})\notag\\
  & \propto \quad \prod_{I \in \partial i } \sumint_{\set{X}_{\partial I
      \back i}} \f_{I}(\x_I) \prod_{j \in \partial I \back i}
  \Ms{j}{I}(\x_j)\label{eq:gsnbp}
\end{align}

Note that \refEq{eq:gsnbp} is identical to BP
estimate of the marginal \refEq{eq:bpmargonly}.  This equality is a
consequence of the way we have defined messages in GS update and
allows us to combine BP and GS updates in the following section.
\end{comment}

\begin{comment}
Here we introduce an alternative to decimation that does not require repeated application of inference.
The basic idea is to use a linear combination of BP and GS operators (\refEq{eq:bpop} and \refEq{eq:gsop}) to update the messages:
\begin{align}
\pbp(\{\Ms{i}{I}\}) \triangleq \gamma \; \gs(\{\Ms{i}{I}\}) + (1 - \gamma) \bp(\{\Ms{i}{I}\})
\end{align}

The Perturbed BP operator $\pbp = \{ \pbpiI{i}{I}\}_{i, I \in \partial i}$ updates each message 
by calculating the outgoing message according to BP and GS operators and linearly combines
them to get the final massage. During $T$ iterations of Perturbed BP, 
the parameter $\gamma$ is gradually and linearly 
changed from $0$ towards $1$. The following algorithm summarizes this procedure.

% We now provide a method to use the stochastic projection procedure above to perturb BP updates.
% Using BP, at any iteration we have an estimate of marginals $\ph_i$.
% We use this estimate to define a sampling distribution $\q_i(\basisp_\ell) := \ph_i(\x_\ell)$ over $\basesp{\set{X}_i}{\gamma}$.
% We then project all the outgoing messages ($\{\Ms{i}{I}\}_{I \in \partial i}$ in \refEq{eq:miI}) to this particular basis.

% In short, we replace all the outgoing messages with their projection into a basis that was chosen according to the estimated local marginal.
% Using $\gamma = 0$, the projection is essentially to a uniform distribution, 
% which produces original BP update. On the other hand, using $\gamma = 1$
% corresponds to Gibbs Sampling (see Appendix A for proof). 
% Perturbed BP starts with $\gamma = 0$ and increases $\gamma$ towards $1$ in each iteration.
% The following summarizes Perturbed BP:

\begin{center}
\line(1,0){300}\\
\textbf{Algorithm:} Perturbed Belief Propagation\\
\line(1,0){300}
\end{center}
\vspace{-.1in}  
\begin{enumerate}\label{perturbedBP}
\item[]\textbf{Input:} factor graph of a CSP, number of iterations T.
\item[]\textbf{Output:} a satisfying assignment $x^*$ if an assignment was found. \emph{UNSATISFIED} otherwise.
\item Initialize messages. 
\item $\gamma \leftarrow 0$.
\\[-1ex]
  \item Repeat $T$ times
  \begin{enumerate}
  \item For each variable $\x_i$:
  \begin{enumerate}
    \item \textbf{Calculate} $\Ms{I}{i}$ using \refEq{eq:mIi} $\forall I \in \partial i$
    \item Return \emph{UNSATISFIED}
if $\{ \Ms{I}{i} \}_{I \in \partial i}$ are contradictory. \label{step:contradictory} 
    \item \textbf{Calculate} $\ph(\x_i)$ using \refEq{eq:gsnbp}. \label{step:calcmarg}
    \item \textbf{Calculate} BP messages $\Ms{i}{I}$ using \refEq{eq:miI}\quad $\forall
    I \in \partial i$.\label{step:calcmessage}
    \item \textbf{Sample} $\xh_i \sim \ph(\x_i)$ \label{step:sample}. 
    \item \textbf{Combine} BP and GS messages:
    $\Ms{i}{I} \; \leftarrow \;  \gamma \  \Ms{i}{I}\  + \ (1 - \gamma)\ \delta(\x_i, \xh_i)$\label{step:projection}
\\[-1ex]
   \end{enumerate}
   \item $\gamma \leftarrow \gamma + \frac{1}{T-1}$ \footnote{We use $T-1$ rather than $T$ 
here to ensure that $\gamma$ is equal to $1$ during the final iteration.}
   \end{enumerate}
\item \textbf{Return} $\x^* = \xh$ as a solution.
\end{enumerate} 
\begin{center}
\line(1,0){300}
\end{center}

In step \ref{step:contradictory}, if the product of incoming messages is $0$ for all $\x_i \in \set{X}_i$ for some $i$,
different neighboring constraints have strict disagreement about
$\x_i$; therefore we can not satisfy this CSP using Perturbed BP.
Since the procedure is inherently stochastic, if the CSP is satisfiable, 
re-application of the same procedure to the problem may avoid
the contradiction. 
\end{comment}

==> chap5.tex <==
\chapter{Conclusions}
    We feel that the novelty in the work lies principally
    in two features: 1) the combination of an exhaustive
    method with a flexible motif representation; and,
    2) the extension of this algorithm to problems
    of a generic nature.  As the reviewer notes,
    the ideas behind these features are drawn
    from a variety of sources --- specifically,
    Teiresias~\citep{rigoutsos1998combinatorial},
    Winnower~\citep{pevzner2000combinatorial}, the
    algorithm by~\cite{mancheron2003pattern};
    and algorithms by~\cite{zaki2000scalable},~\cite{zaki1998theoretical},
    and~\cite{mancheron2003pattern}.  We feel that,
    in addition, there are ideas
    that are introduced for the first time in this
    manuscript.  For example, the convolution algorithm presented
    is unique from that described by~\cite{rigoutsos1998combinatorial} 
    in that it utilizes the offsets of $L$--length windows rather
    than fixed strings.  This slight difference makes
    convolution significantly more difficult and is one
    of the features that allows the Gemoda algorithm to
    discover motifs that cannot be well--represented using
    regular expressions.


==> contents.tex <==
  % -*- Mode:TeX -*-
%% This file simply contains the commands that actually generate the table of
%% contents and lists of figures and tables.  You can omit any or all of
%% these files by simply taking out the appropriate command.  For more
%% information on these files, see appendix C.3.3 of the LaTeX manual. 
\tableofcontents
\newpage
\listoffigures
\newpage
\listoftables



==> convergence.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 
\subsection{Sufficient conditions}
\todo{damping, combining bp updates to get a bp operator}

\subsection{Convergent alternatives}
\begin{comment}
The convergence properties of BP and GBP have been widely studied and many
variations with better properties have been proposed.

Here we first review the main literature on the conditions for convergence of
BP.
For a detailed treatment and experimental comparison of sufficient conditions
for convergence, see \refCite{Mooij2008}.
\refCite{Tatikonda2002} reduced the condition for convergence of BP to
uniqueness of Gibbs measure on a new PGM (called computation tree), constructed
based on BP's message passing 
(see \refSection{sec:bigpicture} for more on Gibbs measure).
% Therefore this result establishes a connection
% between convergence of BP and the general tractability of the corresponding
% inference problem. 
% In
% \refSection{sec:bigpicture} we will intoruce the Gibbs measure and discuss its
% multiplicity with regard to phase transitions to difficult inference regiem.
\refCite{Heskes2004} provides sufficient conditions based on the uniqueness of
 the fixed points of Bethe free energy. This argument is based on the convexity
conditions for the Bethe entropy of \refEq{eq:bethe} and the analysis of the
minimax problem arising from the Lagrangian of \refEq{eq:bethefreeenergy}.
Tighter sufficient conditions are provided by \refCite{Mooij2007a} and
\refCite{Ihler2005a}. Here BP is viewed as an ``operator'' that takes a set of
messages to a new set; the authors provide convergence guarantees, based on
``contraction property'' of this operator--\ie if repeated application will
produce messages that are closer to their predecessor at each iteration. 

One of the main ideas in design of message passing algorithms with better
convergence properties is to find convex relaxations/bounds to
Bethe/Kikuchi free energy and solve the resulting optimization.
Most notably, Tree Reweighted BP defines a distribution on spanning (hyper)
trees embedded in the original loopy PGM (\refCite{Wainwright2005,Wainwright2005a}).
Since the Bethe entropy for each (hyper) tree is convex, the weighted sum remains convex. In
fact, we can rewrite the corresponding entropy approximation as \footnote{The
first term in the summation is the mutual information of variables in one
factor, and this formulation reduces to Bethe entropy of \refEq{eq:bethe}}:
\begin{align}\label{eq:trwentropy}
\ent_{TRW}(\p) \quad = \quad \sum_{\I{I}} \cn(\I{I})
\left ( \ent(\p(\x_{\I{I}})) - \sum_{i \in \I{I}} \ent(\p(\x_i)) \right ) \; +
\; \sum_{i} (\Ne{i} - 1) \ent(\p(\x_i))
\end{align}
 where the counting number $
\cn(\I{I}) \in [0,1]$ is the sum of the weight of the (hyper) trees in which 
the factor $\I{I}$ appears. This results in a message passing procedure very
similar to BP and can be used for both marginalization and MAP inference. 

Another variation is given by Fractional BP, 
which reduces to both BP and Naive MF by changing of a single parameter that
accounts for inclusion of variable interactions into energy approximation (
\refCite{Wiegerinck2003}). 

A family of convergent alternatives of BP is the class of double loop
algorithms that tighten an upper bound on the free energy
(\refCite{Heskes2006,Teh2002,Yuille2002}).
A generalization is given by \refCite{Heskes2006}.

There are variety of other convergent message passing methods --\eg
\refCite{Globerson2007,Meltzer2009,Hazan2008,Kolmogorov2006}--
some of which guarantee convergence for convex free energies (such as that of
\refEq{eq:trwentropy}) under particular update schedule.

The research on MAP inference has followed two other
directions in addition what we have already discussed
\begin{itemize}
  \item  MAP inference can also be
formulated using Linear Programming relaxations. 
The corresponding optimization has close connections to max-product BP and zero
temperature limits of sum-product BP (\refCite{Koller2009,Weiss2007}). Some
efforts have been focused on closing the gap between LP (and quadratic programming)
relaxations and max-product (\eg
\refCite{Yanover2006,Weiss2011,Globerson2007}).

\item The other active area is energy minimization using graph-cuts 
--with applications mainly within image
processing \refCite{Demetz2009,Boykov2001}-- which has a close connections to MAP inference
(\refCite{Tarlow2011}) and can provide optimal solutions to
optimization problems with restricted form of factors (\ie regular potentials).
\end{itemize}
\end{comment}

==> cover.tex <==
% -*-latex-*-
% $Log: cover.tex,v $
% Revision 1.7  2001/02/08 18:53:16  boojum
% changed some \newpages to \cleardoublepages
%
% Revision 1.6  1999/10/21 14:49:31  boojum
% changed comment referring to documentstyle
%
% Revision 1.5  1999/10/21 14:39:04  boojum
% *** empty log message ***
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.3  93/05/17  17:06:29  starflt
% Added acknowledgements section (suggested by tompalka)
% 
% Revision 1.2  92/04/22  13:13:13  epeisach
% Fixes for 1991 course 6 requirements
% Phrase "and to grant others the right to do so" has been added to 
% permission clause
% Second copy of abstract is not counted as separate pages so numbering works
% out
% 
% Revision 1.1  92/04/22  13:08:20  epeisach
\addcontentsline{toc}{chapter}{Cover page}
\title{Message Passing for Combinatorial Optimization}
\author{Siamak Ravanbakhsh}
\department{Department of Computing Science}
% If the thesis is for two degrees simultaneously, list them both
% separated by \and like this:
 \degree{Doctor of Philosophy}
%\degree{Bachelor of Science in Computer Science and Engineering}
\degreemonth{Sep}
\degreeyear{2014}
\thesisdate{Aug 27, 2014}

%% By default, the thesis will be copyrighted to MIT.  If you need to copyright
%% the thesis to yourself, just specify the `vi' documentclass option.  If for
%% some reason you want to exactly specify the copyright notice text, you can
%% use the \copyrightnoticetext command.  
\copyrightnoticetext{\copyright ~Siamak Ravanbakhsh, 2014.}

\begin{comment}
\copyrightnoticetext{\copyright ~Siamak Ravanbakhsh, 2014. \\
{\footnotesize
This work is licensed under the Creative
Commons Attribution-NonCommercial 2.5
License. To view a copy of this license, visit
\url{http://creativecommons.org/licenses/by-nc/2.5/} or send a
letter to
Creative Commons
543 Howard Street, 5th Floor,
San Francisco, California, 94105, USA.
}}
\end{comment}

% If there is more than one supervisor, use the \supervisor command
% once for each.
\supervisor{Russell Greiner}{Professor of Computing Science}

% This is the department committee chairman, not the thesis committee
% chairman.  You should replace this with your Department's Committee
% Chairman.
%\chairman{Daniel Blankschtein}{Chairman, Department Committee on Graduate Students}
\chairman{XXXX}{Chairman, Department Committee on Graduate Students}

% Make the titlepage based on the above information.  If you need
% something special and can't use the standard form, you can specify
% the exact text of the titlepage yourself.  Put it in a titlepage
% environment and leave blank lines where you want vertical space.
% The spaces will be adjusted to fill the entire page.  The dotted
% lines for the signatures are made with the \signature command.
\maketitle

% The abstractpage environment sets up everything on the page except
% the text itself.  The title and other header material are put at the
% top of the page, and the supervisors are listed at the bottom.  A
% new page is begun both before and after.  Of course, an abstract may
% be more than one page itself.  If you need more control over the
% format of the page, you can use the abstract environment, which puts
% the word "Abstract" at the beginning and single spaces its text.

%% You can either \input (*not* \include) your abstract file, or you can put
%% the text of the abstract directly between the \begin{abstractpage} and
%% \end{abstractpage} commands.

% First copy: start a new page, and save the page number.
\cleardoublepage
% Uncomment the next line if you do NOT want a page number on your
% abstract and acknowledgments pages.
\pagestyle{empty}
\setcounter{savepage}{\thepage}
\begin{abstractpage}\addcontentsline{toc}{chapter}{Abstract}
\input{abstract}
\end{abstractpage}

% Additional copy: start a new page, and reset the page number.  This way,
% the second copy of the abstract is not counted as separate pages.
% Uncomment the next 6 lines if you need two copies of the abstract
% page.
% \setcounter{page}{\thesavepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

\cleardoublepage

\section*{Acknowledgments}\addcontentsline{toc}{chapter}{Acknowledgments}

\todo{ack goes here...}
% I am indebted to many people who both directly and indirectly
% contributed to this thesis.  First, I would like to thank those
% collaborators who directly contributed.  Most of all, I'm grateful
% for the help and friendship of Mark Styczynski. Mark was my
% collaborator on all matters computational for the past four years
% --- his influence is evident throughout this document.  I'm also
% grateful for my collaboration with Christopher Loose, who performed
% many of the experiments on antimicrobial peptides described in
% Chapter~\ref{chapter:amps}.  Finally, I would like to thank Isidore Rigoutsos, who
% straddled the line between collaborator and advisor.  Isidore taught
% me an attention to detail and a penchant for the UNIX command line
% and vi editor.

% Most importantly, I am indebted to Greg Stephanopoulos, my advisor,
% whose guidance and support was unwavering these past six years. Greg
% is the perpetual optimist --- always positive in the face of my many
% failures along the way.  He also gave me the freedom to pursue
% projects of my own choosing, which contributed greatly to my
% academic independence, if not the selection of wise projects.

% I am much obliged to my thesis committee members: my advisor Greg,
% Isidore, Bill Green, and Bob Berwick.  My committee was always
% flexible in scheduling and judicious in their application of both
% carrots and sticks.

% There are numerous people who contributed indirectly to this thesis.
% First among these is my intelligent, lovely, and vivacious wife
% Kathryn Miller--Jensen.  Next, my parents Carl and Julie, my sister
% Heather, and my in-laws, Ron, Joyce, Suzanne, Jeff, and Mindi.
% Finally, there are innumerable friends who contributed and to whom I
% am greatly appreciative including Michael Raab, Joel Moxley, Bill
% Schmitt, Vipin Guptda, and Jatin Misra.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -*-latex-*-


==> glossaries.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 



==> packing.tex <==
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


\begin{comment}%complexity
\noindent \textbf{K-Packing (binary variable):}\\
The time complexity of Perturbed BP iterations in this factor-graph is
dominated by factor-to-variable messages sent from $\f_{\K}(\x)$ to
all variables.  Assuming asynchronous update, the complexity for
min-max procedure is $\set{O}(N^2 K \log(N))$.

\noindent \textbf{K-Packing (categorical variable):}\\
Since the factors are not sparse, the complexity of factor-to-variable
messages are $\set{O}(N^2)$, resulting in $\set{O}(N^2K^2)$ cost per
iteration for $\p_{\y}$-reduction.  Since the diversity of pairwise
distances is $|\set{Y}| = \set{O}(N^2)$, the general cost of finding
an approximate min-max solution by message passing is $\set{O}(N^2K^2
\log(N))$.

\noindent \textbf{Sphere-Packing (Hamming distance):}\\
The total number of variables (including $x$ and $z$) in this
factor-graph is $N = K n + \frac{K (K-1)}{2} n = \set{O}(n K^2)$.  The
factor-graph contains $\frac{K (K-1)}{2} n$ z-factors and $\frac{K
  (K-1)}{2}$ distance factors.  Each $x_{i-k}$ variable receives
messages from $K-1$ z-factors while each $z(i,j)_k$ variable is
connected to one z-factor and one distance factor.  Assuming an
asynchronous message update the cost of factor-to-variable messages
from distance-factors (\ie $\set{O}(n^2y)$) dominates the complexity
of Perturbed BP's iterations.  Since there are $K^2$ such factors the
complexity of message passing per iteration is $\set{O}(K^2n^2y)$.
\end{comment}

\begin{comment}
Given a symmetric distance matrix $D \in \Re^{N \times N}$ between $N$
data-points and a number of code-words $K$, the $K$-packing problem is
to choose a subset of $K$ points such that the minimum distance
$D_{i,j}$ between any two code-words is maximized.  Here we introduce
two different factor-graph formulations for this problem.

\subsubsection{First Formulation: Binary Variables}\label{sec:packing_binary}
Let binary variables $\x = \{ \x_1,\ldots,\x_N\} \in \{0,1\}^{N}$,
indicate a subset of variables of size $K$ that are selected as
code-words (\refFigure{fig:kpackbin_fg}).  Use the factor
$\f_{\K}(\x) = \infty\I(\sum_{i}\x_i \neq K) -\infty \I(\sum_{i}\x_i
= K)$ (here $\K = \{1,\ldots,N\}$) to ensure this constraint.  The
$\p_{y}$-reduction of this factor for any $-\infty < y < +\infty$ is a
K-of-N factor as defined in \refSection{sec:hop}.  Furthermore, for
any two variables $\x_i$ and $\x_j$, define factor
$\f_{\x_i,\x_j}(\x_{i,j}) = -D_{i,j}\x_i\x_j - \infty(1 -
\x_i\x_j)$. This factor is effective only if both points are selected
as code-words. The use of $-D_{i,j}$ is to convert the initial max-min
objective to min-max.

\subsubsection{Second Formulation: Categorical Variables}\label{sec:packing_categorical}
Define the K-packing factor-graph as follows: Let $\x = \{
\x_1,\ldots, \x_K\}$ be the set of variables where $\x_i \in \set{X}_i
= \{1,\ldots,N\}$ (\refFigure{fig:kpackcat_fg}).  For every two
distinct points $1 \leq i <j \leq K$ define the factor
$\f_{\{i,j\}}(\x_i,\x_j) = -D_{\x_i,\x_j} \I(\x_i \neq \x_j) +\infty
\I(\x_i = \x_j)$. Here each variable represents a code-word and the
last term of each factor ensures that code-words are distinct.

\begin{proposition}\label{th:packing}
  The $\p_{\y}$-reduction of the $K$-packing factor-graph for the distance
  matrix $D \in \Re^{N \times N}$ defines a uniform distribution over
  the cliques of $\set{G}(-D, -y)$ that are larger than $K$.
\end{proposition}
The $\p_{\y}$-reduction of our second formulation is similar to the
factor-graph used by \refCite{ramezanpour2012cavity} to find
non-linear binary codes.  The authors consider the Hamming distance
between all binary vectors of length $n$ (\ie $N = 2^n$) to obtain
binary codes with known minimum distance $y$. As we saw, this method
is $\set{O}(N^2K^2) = \set{O}(2^{2n}K^2)$ --\ie grows exponentially
in the number of bits $n$. In the following section, we introduce a
factor-graph formulation specific to categorical variables with
Hamming distance that have message passing complexity
$\set{O}(n^2K^2y)$ --\ie not exponential in $n$. Using this
formulation we find optimal binary codes where both $n$ and $y$ are
large.

\subsubsection{Efficient packing with Hamming distance}\label{sec:hamming}
Our factor-graph defines a distribution over the $K$ binary vectors of
length $n$ such that the distance between every pair of binary vectors
is at least $y$.\footnote{ For convenience we restrict this
  construction to the case of binary vectors.  A similar procedure may
  be used to find maximally distanced ternary and $q$-ary vectors, for
  arbitrary $q$.}  Finding so-called ``nonlinear binary codes'' is a
fundamental problem in information theory and a variety of methods have
been used to find better codes, trying either to maximize the number of keywords $K$
or their minimum distance $y$ (\eg see
\refCitep{bincodes} and its references).
\begin{figure}
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/packing_euclidean.pdf}
  \end{minipage}
  \hspace{-.02\linewidth}
  \begin{minipage}[b]{0.2\linewidth}
    \centering \scalebox{.4}{
      \begin{tabular}[b]{cccccccccccccccc}
        2& 1& 2& 1& 0& 1& 1& 2& 2& 1& 2& 1& 2& 1& 0& 2\\
        1& 1& 1& 2& 1& 0& 0& 2& 2& 1& 1& 1& 0& 2& 1& 0\\
        0& 0& 1& 2& 0& 1& 2& 0& 2& 1& 2& 2& 1& 0& 2& 0\\
        0& 0& 0& 2& 1& 0& 1& 2& 1& 0& 1& 0& 2& 1& 0& 1\\
        2& 2& 0& 2& 2& 2& 1& 1& 2& 0& 2& 2& 1& 2& 1& 2\\
        0& 2& 0& 0& 0& 2& 0& 2& 0& 0& 2& 1& 0& 0& 0& 0\\
        1& 1& 2& 0& 0& 1& 2& 2& 0& 0& 1& 0& 1& 2& 2& 1\\
        2& 0& 2& 0& 2& 1& 0& 1& 1& 2& 0& 1& 1& 1& 2& 0\\
        0& 2& 1& 1& 1& 1& 1& 1& 0& 1& 0& 0& 0& 0& 1& 2\\
        1& 0& 0& 1& 0& 2& 0& 0& 1& 2& 0& 0& 2& 2& 1& 2\\
        1& 2& 2& 1& 1& 0& 2& 1& 1& 2& 2& 2& 2& 0& 2& 1\\
        1& 0& 1& 0& 2& 2& 2& 1& 0& 1& 1& 2& 2& 1& 0& 2\\
      \end{tabular}
    }
  \end{minipage}
  \vspace{-.18in}
  \caption{\small{\textbf{(left)} Using message passing to choose $K =
      30$ out of $N = 100$ random points in the Euclidean plane to
      maximize the minimum pairwise distance (with $T = 500$
      iterations for PBP). Touching circles show the minimum distance.
      \textbf{(right)} Example of an optimal ternary code ($n = 16,
      y=11, K=12$), found using the K-packing factor-graph of
      \refSection{sec:hamming}.  Here each of $K = 12$ lines contains
      one code-word of length $16$, and every pair of code-words are
      different in at least $y = 11$ digits.}}\label{fig:ternary}
\end{figure}
\vspace{-.1\in} Let $\x = \{\x_{1-1}, \ldots,\x_{1-n},
\x_{2-1},\ldots,\x_{2-n},\ldots,\x_{K-n}\}$ be the set of our binary
variables, where $\x_i = \{\x_{i-1},\ldots,\x_{i-n}\}$ represents the
$i^{th}$ binary vector or code-word.  Additionally for each $ 1\leq i
< j \leq K$, define an auxiliary binary vector $z_{i,j} = \{ z_{i,j,1},\ldots,z_{i,j,n}\}$ of length $n$ (\refFigure{fig:spherepack_fg}).

For each distinct pair of binary vectors $x_{i}$ and $x_j$, and a particular
bit $1 \leq k \leq n$, the auxiliary variable $z_{i,j,k} = 1$
\emph{iff} $x_{i-k} \neq x_{j-k}$.  Then we define an
at-least-$y$-of-$n$ factor over $z_{i,j}$ for every pair of code-words,
to ensure that they differ in at least $y$ bits.

In more details, define the following factors on $\x$ and $z$:\\
(a) \textit{z-factors:} For every $ 1\leq i < j \leq K$ and $1 \leq k
\leq n$, define a factor to ensure that $z_{i,j,k} = 1$ \emph{iff}
$x_{i-k} \neq x_{j-k}$:
\begin{align*}
  \f(\x_{i-k},\x_{j-k},z_{i,j,k}) &= 
                                   \I(\x_{i-k} \neq \x_{j-k})\I(z_{i,j,k} = 1)\\& + \I(\x_{i-k} = \x_{j-k})\I(z_{i,j,k} = 0).
\end{align*}
This factor depends on three binary variables, therefore we can
explicitly define its value for each of $2^3 = 8$ possible inputs.

(b) \textit{distance-factors:} For each $z_{i,j}$ define
at-least-y-of-n factor:
\begin{align*}
  \f_{\K}(z_{i,j}) = \I(\sum_{1\leq k \leq n} z_{i,j,k} \geq y)
\end{align*}

\refTable{table:binarycode} reports some optimal codes including codes
with large number of bits $n$, recovered using this factor-graph. Here
Perturbed BP used $T = 1000$ iterations.
\begin{table}
  \caption{\small{Some optimal binary codes from \refCitep{bincodes} 
      recovered by K-packing factor-graph
      in the order of increasing $y$.
      $n$ is the length of the code, $K$ is the number of code-words and $y$
      is the minimum distance between code-words.}}\label{table:binarycode}

  \scalebox{.7}{
    \begin{tabular}{|r|c|l||r|c|l||r|c|l || r|c|l |}
      \hline
      n & K & y & n & K & y &n & K & y &n & K & y\\\hline\hline
      8 & 4& 5 &11 &4 &7 &14 &4 &9 &16 &6 &9 \\\hline
      17 & 4 & 11 &19 &6 &11 &20 &8 &11 &20 &4 &13 \\\hline
      23 & 6 & 13 &24 &8 &13 & 23&4 &15 &26 & 6& 15\\\hline
      27 & 8 & 15 &28 &10 &15 &28 &5 &16 &26 &4 &17 \\\hline
      29 & 6 & 17 &29 &4 &19 &33 &6 & 19&34 &8 &19 \\\hline
      36 & 12 & 19 &32 &4 &21 &36 &6 &21 &38 &8 &21 \\\hline
      39 &10  &21  &35 & 4& 23& 39& 6&23 & 41& 8&23 \\\hline
      39 &4  &25  & 43& 6&23 &46 &10 &25 &47 &12 &25 \\\hline
      41 & 4 &27  & 46& 6& 27&48 &8 &27 &50 &10 &27 \\\hline
      44 & 4 &29  &49 & 6& 29& 52&8 &29 &53 &10 &29 \\\hline
    \end{tabular}
  }
\end{table}

\begin{figure*}
  \centering \hbox{ \subfigure[]{
      \label{fig:mmclust_fg}\label{fig:btsp_fg}\label{fig:kpackcat_fg} \includegraphics[width=.18\textwidth]{figures/mmclust.pdf}
    } \subfigure[K-packing (binary)]{
      \includegraphics[width=.18\textwidth]{figures/kpackbinary.pdf}
      \label{fig:kpackbin_fg}
    } \subfigure[sphere packing]{
      \includegraphics[width=.27\textwidth]{figures/spherepack.pdf}
      \label{fig:spherepack_fg}
    } \subfigure[K-center]{
      \includegraphics[width=.27\textwidth]{figures/kcenter.pdf}
      \label{fig:kcenter_fg}
    } } \vspace{-.2in}
  \caption{\small{The factor-graphs for different
      applications. Factor-graph (a) is common between min-max
      clustering, Bottleneck TSP and K-packing (categorical). However
      the definition of factors is different in each case.}}
\end{figure*}

\begin{proof}\ref{th:packing}
  Here we prove Proposition~\ref{th:packing} for the factor-graph of
  \refSection{sec:packing_categorical}.  The proof for the binary
  variable model follows the same procedure.  Since $\p_\y$ defines a
  uniform distribution over its support, it is enough to show that any
  clique of size $K$ over $\set{G}(-D,-y)$ defines a unique set of
  assignments all of which have nonzero probability ($\p_\y(\x) > 0$)
  and any assignment $\x$ with $\p_\y(\x) > 0$ defines a unique clique
  of size at least $K$ on $\set{G}(-D, -y)$.  First note that the
  basic difference between $\set{G}(D, y)$ and $\set{G}(-D, -y)$ is
  that in the former all nodes that are connected have a distance of
  at most $y$ while in the later all nodes that have a distance of at
  least $y$ are connected to each other.  Consider the
  $\p_\y$-reduction of the pairwise factors of the factor-graph
  defined in \refSection{sec:packing_categorical}:
  \begin{align}\label{eq:packing_reduction}
    \f^\y_{\{i,j\}}(\x_i,\x_j) =  \I(\x_i \neq \x_j \wedge -D_{\x_i,\x_j} \leq y)
  \end{align}

  \emph{(A) Any clique of size $K$ in $\set{G}(-D, -y)$, defines $K\!$
    unique assignments, such that for any such assignment $x$,
    $\p_\y(\x) > 0$:}
  % Recall that $\x = \{ x_1,\ldots,\x_K\}$ represent code-words where
  % $\x_i \in \{1,\ldots,N\}$.
  For a clique $\set{C} = \{c_1,\ldots,c_K\}$ of size $K$, define $x_i
  = c_{\pi(i)}$, where $\pi: \{1,\ldots,K \} \to \{1,\ldots,K \}$ is a
  permutation of nodes in clique $\set{C}$. Since there are $K\!$ such
  permutations we may define as many assignments $x$.  Now consider
  one such assignment $x$.  For every two nodes $x_i$ and $x_j$, since
  they belong to the clique $\set{C}$ over $\set{G}(-D, -y)$, they are
  connected and $D_{x_i, \x_j} \geq y$. This means that all the
  pairwise factors defined by \refEq{eq:packing_reduction} have
  non-zero values and therefore $\p_\y(x) > 0$.

  \emph{(B) Any assignment $x$ with $\p_\y(\x) > 0$ corresponds to a
    unique clique of size $K$ in $\set{G}(-D,-y)$:} Let $\set{C} =
  \{x_1, \ldots, \x_K\}$. Since $\p_\y(\x) > 0$, all pairwise factors
  defined by \refEq{eq:packing_reduction} are non-zero.  Therefore
  $\forall i,j\neq i\;\; D_{\x_, \x_j} \geq y$, which means all $x_i$
  and $x_j$ are connected in $\set{G}(-D,-y)$, forming a clique of
  size $K$.
\end{proof}

\end{comment}

==> permutations.tex <==

\subsection{Matching and Permanent}\label{sec:matching}
\subsection{Isomorphism and symmetries}\label{sec:isomorphism}
\subsection{Traveling salesman problem}\label{sec:tsp}
\input{tsp.tex}
